Cloud Gaming With Foveated Graphics

Cloud gaming enables playing high end games, originally designed for PC or game console setups, on low end devices, such as net-books and smartphones, by offloading graphics rendering to GPU powered cloud servers. However, transmitting the high end graphics requires a large amount of available network bandwidth, even though it is a compressed video stream. Foveated video encoding (FVE) reduces the bandwidth requirement by taking advantage of the non-uniform acuity of human visual system and by knowing where the user is looking. We have designed and implemented a system for cloud gaming with foveated graphics using a consumer grade real-time eye tracker and an open source cloud gaming platform. In this article, we describe the system and its evaluation through measurements with representative games from different genres to understand the effect of parameterization of the FVE scheme on bandwidth requirements and to understand its feasibility from the latency perspective. We also present results from a user study. The results suggest that it is possible to find a "sweet spot" for the encoding parameters so that the users hardly notice the presence of foveated encoding but at the same time the scheme yields most of the bandwidth savings achievable.

==> related_work.tex <==
\section{Related Work}
\label{sec:related}



Although there have been investigations into QoE of cloud gaming, for example, \cite{Jarschel_Qoe}, to the best of our knowledge, foveated video streaming for cloud gaming and its QoE has not been investigated. 
Many works have studied QoE in foveated video encoding and imaging, however, since there a standard foveated encoding does not exist, the parameters considered are different from the parameter we consider.
%Finally, many papers have been published on different kinds of gaze tracking solutions~\cite{shimizu16ubicomp,greenwald16vrst,geiselhart16ubicomp}.
%From Tuomas's 
. % The software in our experiments does not directly allow for modulating the magnitude of distortions in the peripheral view, but we can assume for now that it is indirectly controlled through the maximum quantization level. Furthermore, we saved the gaze streaming data from our experiments, which would allow us to simulate Rai et al.'s approach and explore a possible relationship between the participant's ratings and their gaze disruptions as an objective metric of video quality.
